Input-Output Stability of Gradient Descent: A Discrete-Time Passivity-Based Approach

This paper presents a discrete-time passivity-based analysis of the gradient descent method for a class of functions with sector-bounded gradients. Using a loop transformation, it is shown that the gradient descent method can be interpreted as a passive controller in negative feedback with a very strictly passive system. The passivity theorem is then used to guarantee input-output stability, as well as the global convergence, of the gradient descent method. Furthermore, provided that the lower and upper sector bounds are not equal, the input-output stability of the gradient descent method is guaranteed using the weak passivity theorem for a larger choice of step size. Finally, to demonstrate the utility of this passivity-based analysis, a new variation of the gradient descent method with variable step size is proposed by gain-scheduling the input and output of the gradient.

==> Sections/0_rough_draft.tex <==
\section{Rough draft}
    \subsection{The Six Questions}
    \begin{itemize}
        \item{%
            What's the problem?
            \\
            \textcolor{blue}{%
                Existing control interpretation of optimization algorithm approaches focus on fixed stepsizes. (exceptions: Analysis of Gradient Descent with Varying Step Sizes using Integral Quadratic Constraints)
            }%
        }%
        \item{%
            Why's this problem important to solve?
            \\
            \textcolor{blue}{%
                In practice, varying stepsizes are used to improve convergence speed.
            }%
        }%
        \item{%
            What are the state of the art solutions (if they exist)?
            \\
            \textcolor{blue}{%
                Analysis of Gradient Descent with Varying Step Sizes using Integral Quadratic Constraints: where the convergence rate guaranteeing global convergence was found to be slower than fixed step size!
            }%
        }%
        \item{%
            What are the deficiencies of the state of the art solutions (if they exist)?
            \\
            \textcolor{blue}{%
                for \(1 \leq c \leq 2\) :
                \(\frac{1}{cL} \leq \alpha_k \leq \frac{c}{L}\) 
            }%
        }%
        \item{%
            What are you proposing to solve the problem? Will your proposed solution address the state of the art solutions' deficiencies?
            \\
            \textcolor{blue}{%
                First show gradient descent algorithm can be interpreted as a passive controller in negative feedback with a VSP system. Then use existing gain-scheduling theorems to mimic the LPV Gradient descent as a gain-scheduled passive controller.
            }%
            \\
            \textcolor{Red}{%
                Bonus: Introducing a new gradient decent algorithm + gradient descent with feedthrough (if space permits)
            }%
        }%
        \item{%
            What evidence do you have that you've actually solved the problem better than (or addressing the deficiencies of) the existing state of the art solutions?
            \\
            \textcolor{blue}{
                Hard core I/O + violin/histogram plots
            }
        }%
    \end{itemize}
    \newpage
    \hspace*{5pt}
    \newpage
    % \subsection{Passivity of GD}
    % Passivity and losslessness of discrete-time systems having outputs independent of \(\mbf{u}_k\) (i.e. \(\mbf{D}=\mbf{0}\)) cannot be studied~\cite{Byrnes_Lin_Losslessness}.
    % \begin{lemma}
        
    % \end{lemma}
    % \newpage
    % \hspace*{5pt}
    % \newpage
    % \subsection{Loop Transformation}
    % \subsection{Impact on Loop Transformation on VSP}
    % \subsection{Gain-Scheduling}
    % \subsection{Comparison with Other Methods}





